Combining dependency, grades, and adjoint logic

We propose two new dependent type systems. The first, is a dependent graded/linear type system where a graded dependent type system is connected via modal operators to a linear type system in the style of Linear/Non-linear logic. We then generalize this system to support many graded systems connected by many modal operators through the introduction of modes from Adjoint Logic. Finally, we prove several meta-theoretic properties of these two systems including graded substitution.

==> dmGL-typing-ottput.tex <==
\subsection*{Typing Rules}

Terms of graded types are denoted by $ \dmGLnt{t} $ and
typing judgments in the graded subsystem have the form $ \delta  \odot  \Delta  \vdash_\mathsf{G}  \dmGLnt{t}  \dmGLsym{:}  \dmGLnt{X} $.
We will not make explicit the grammar of graded terms,
it should be easy to read off from the typing rules below.
Terms in the mixed system are denoted by $ \dmGLnt{l} $ and the judgment form
mixed typing judgments is $ \delta  \odot  \Delta  \dmGLsym{;}  \Gamma  \vdash_\mathsf{M}  \dmGLnt{l}  \dmGLsym{:}  \dmGLnt{A} $.
Again, we omit the grammar for terms in the mixed system.

\begin{atom}[Type Formation]
  We first explain how types are formed in our system.
  \dmGL{} has a universe $ \mathsf{Type} $ of graded types
  and a universe $ \mathsf{Linear} $ of linear types,
  which are both themselves graded types.
  This is because we want to allow for linear types to depend on variables of graded types.
  The rules for type formation are given in \Cref{fig:typeFormation}.
\end{atom}


\begin{figure}
  \begin{mdframed}
    \pprules[G]{type,linear,unit,function,gradedPair,coproduct,linearFunction,tensor,ladj,radj}
  \end{mdframed}
  \caption{Rules for type well-formedness}
  \label{fig:typeFormation}
\end{figure}


\begin{atom}[Graded Subsystem]
  Graded typing judgments have the form $ \delta  \odot  \Delta  \vdash_\mathsf{G}  \dmGLnt{t}  \dmGLsym{:}  \dmGLnt{X} $.
  Graded typing judgments can be weakened provided the new variable
  is used with grade $ 0 $.
  Similarly for the variable rule,
  the ``returned'' variable must used with grade $ 1 $
  while all other variables are used with grade $ 0 $.
  We also include a subusaging rule,
  which asserts that we can make judgments with higher grades than necessary.
  \pprules[G]{var,weak,subusage}
  The graded unit type $ \mathbf{J} $ has one closed constructor $ \mathbf{j} $
  and its terms can be eliminated at any grade:
  \pprules[G]{unitIntro, unitElim}
  The coproduct type has the expected left and right injections.
  To eliminate a term of the coproduct $ \dmGLnt{X_{{\mathrm{1}}}}  \boxplus  \dmGLnt{X_{{\mathrm{2}}}} $
  it is necessary to specify dependent terms over $ \dmGLnt{X_{{\mathrm{1}}}} $
  and $ \dmGLnt{X_{{\mathrm{2}}}} $ with the caveat that these dependent terms must use the same grades
  and the variable of type $ \dmGLnt{X_{\dmGLmv{i}}} $ ($ i \in \{1,2\} $)
  must be used with grade at least $ 1 $.
  \todom{why at least 1? (something semantic I think?)}
  \pprules[G]{coproduct, coproductInl, coproductInr, coproductElim}
  The dependent function type $ (  \dmGLmv{x}  :^{ \dmGLnt{r} }  \dmGLnt{X}  )  \to   \dmGLnt{Y} $
  comes with a grade annotation $ \dmGLnt{r} $
  specifying with what grade the argument a function has to be used.
  As usual, functions are introduced by lambda abstraction
  and elminated by application.
  The grade annotation corresponds to the grade used in the context.
  \pprules[G]{lambda,app}
  Like the dependent function type,
  the graded pair type also comes with a grade annotation.
  In this case though, the annotation $ \dmGLnt{r} $ means that the
  first component of the pair must be used $ \dmGLnt{r} $ times as often as the second component.
  The rules are thus:
  \pprules[G]{gradedPairIntro,gradedPairElim}
\end{atom}


\begin{atom}[Mixed Subsystem]
  Mixed typing judgments have the form
  $ \delta  \odot  \Delta  \dmGLsym{;}  \Gamma  \vdash_\mathsf{M}  \dmGLnt{l}  \dmGLsym{:}  \dmGLnt{A} $.
  The rules of the mixed fragment strongly resemble linear logic.
  In each rule, all the hypotheses share the same graded context,
  with possibly differing grade vectors, so the mixed fragment can be thought of
  as linear logic where additional variables from the graded context are available.
  Concatenation of linear contexts corresponds to addition of grade vectors in the graded section.
  The mixed typing rules are given in \Cref{fig:mixedTyping}.
\end{atom}


\begin{figure}
  \begin{mdframed}
    \pprules[M]
    {id, exchange, unitIntro, unitElim, lambda, app, tensorIntro, tensorElim}
  \end{mdframed}
  \caption{Mixed Typing Rules}
  \label{fig:mixedTyping}
\end{figure}


\begin{atom}[Modalities]
  \label{atom:dmGLmodalities}
  \dmGL{} includes modal operators $ \mathcal{F} $ and $ \mathcal{G} $ mediating
  between the graded and mixed subsystems.
  The design of these resembles the adjoint operators in Krishnaswami's dependent system
  \cite{Krishnaswami2015}.
  The right adjoint $ \mathcal{G} $ takes a linear type $ \dmGLnt{A} $
  and produces a graded type $ \mathcal{G} \, \dmGLnt{A} $.
  The introduction and elimination rules allow us to convert
  between terms of $ \dmGLnt{A} $ over an empty linear context,
  and terms of $ \mathcal{G} \, \dmGLnt{A} $.
  \todom{Do we want a rule asserting that $ \mathcal G^{-1} \, \mathcal{G} \, \dmGLnt{l} $ is equal to $ \dmGLnt{l} $?}
  {\small
    \begin{mathpar}
      \namedrule[G]{radjIntro}
      \and
      \namedrule[M]{radjElim}
    \end{mathpar}
  }
  The left adjoint $ \mathcal{F}  ( \dmGLmv{x}  :^{ \dmGLnt{r} }  \dmGLnt{X} ). \dmGLnt{A} $ is a linear type
  which behaves like a dependent pair type,
  in which the first component of the pair is a graded term
  and the second component is a linear term.
  The grading annotation $ \dmGLnt{r} $ has a similar role as the annotation
  for graded dependent pair types.
  Terms of this type are introduced by a pairing constructor,
  and eliminated by pattern matching on pairs
  where the first graded component must be used with grade $ \dmGLnt{r} $.

  \[
    \small
    \namedrule[M]{ladjIntro}
    \;\;
    \namedrule[M]{ladjElim}
  \]
\end{atom}


==> fullspec-ottput.tex <==
\drules[G]{$\delta  \odot  \Delta  \vdash_\mathsf{G}  \dmGLnt{t}  \dmGLsym{:}  \dmGLnt{X}$}{test}{%
  var,subusage
}

